URECA: Unique Region Caption Anything

Region-level captioning aims to generate natural language descriptions for specific image regions while highlighting their distinguishing features. However, existing methods struggle to produce unique captions across multi-granularity, limiting their real-world applicability. To address the need for detailed region-level understanding, we introduce URECA dataset, a large-scale dataset tailored for multi-granularity region captioning. Unlike prior datasets that focus primarily on salient objects, URECA dataset ensures a unique and consistent mapping between regions and captions by incorporating a diverse set of objects, parts, and background elements. Central to this is a stage-wise data curation pipeline, where each stage incrementally refines region selection and caption generation. By leveraging Multimodal Large Language Models (MLLMs) at each stage, our pipeline produces distinctive and contextually grounded captions with improved accuracy and semantic diversity. Building upon this dataset, we present URECA, a novel captioning model designed to effectively encode multi-granularity regions. URECA maintains essential spatial properties such as position and shape through simple yet impactful modifications to existing MLLMs, enabling fine-grained and semantically rich region descriptions. Our approach introduces dynamic mask modeling and a high-resolution mask encoder to enhance caption uniqueness. Experiments show that URECA achieves state-of-the-art performance on URECA dataset and generalizes well to existing region-level captioning benchmarks.

==> figs/previous_methods.tex <==
\begin{figure}[t]
    \centering
    \vspace{-15pt}
    \includegraphics[width=\linewidth]{figs/files/yellow_gogo.png}
    \vspace{-10pt}
    % \caption{Pipelines of previous works (a) and proposed \ours pipeline (b).}
    \caption{\textbf{Comparison between (a) previous approaches and (b) proposed \ours framework.}}
    \vspace{-10pt}
    \label{fig:previous}
\end{figure}

==> figs/teaser.tex <==
\begin{figure*}[ht]
    \centering
    \includegraphics[width=\linewidth]{figs/files/ureca_teaser.pdf}
    \caption{\textbf{Overall pipeline of the proposed framework, \ours.} .}
    \label{fig:main_figure}
\end{figure*}

==> sec/1_intro.tex <==
\section{Introduction}
\label{sec:intro}
Multi-granularity region-level captioning aims to describe any specific region in natural language while highlighting its unique features compared to other regions. It remains a challenging task~\cite{DenseCap, kosmos-2, glamm, Yu_2017_CVPR, osprey, controlcap, sca, omg-llava} due to key challenges that include effectively localizing the user-intended region and capturing its unique attributes~\cite{wang2020uniqueinformativecaptioningimages, liu2019generating, wang2020compare} (e.g. color, relative position, and shape) to differentiate it from surrounding regions. Furthermore, it remains difficult to generate unique captions~\cite{Pseudo-RIS, refcap} for regions of any granularity, as most previous studies have focused on prominent regions. Although multimodal language models (MLLM)~\cite{internvl-25, llava, improvedllava, arcana} have been explored for this task, they still struggle to produce truly unique captions due to limitations in both model design and dataset availability.

% Vision-Language Models (VLMs) have attracted significant attention due to their strong performance in region-level understanding and captioning tasks. Although the captions generated by VLMs describe regions well, they often struggle to produce distinctive captions~\cite{yu2024pseudo} conditioned on various levels of region granularity. This limitation makes it difficult for users to accurately indicate the corresponding regions with the generated captions. While VLMs have demonstrated impressive results in image-level captioning, generating distinctive captions for multi-granular regions within an image remains a challenging task.

Previous approaches~\cite{grit, flexcap, groma, gpt4roi} have explored regional captioning by providing region coordinates through natural language descriptions~\cite{llava, minigpt}, marking regions directly on the image (e.g., mask contours, ellipses, bounding boxes, triangles, scribbles, points, arrows, and masks)~\cite{vip-llava, yang2023finegrainedvisualprompting, shtedritski2023doesclipknowred}, or utilizing visual RoI features~\cite{regiongpt, omni-rgpt}. However, they come with several drawbacks: they may alter the original image, make it difficult to distinguish between colored contours, and fail to capture global relationships within the image~\cite{alpha-clip}, ultimately hindering the model's ability to generate accurate and unique captions.

In addition, existing captioning datasets~\cite{groma, osprey, glamm, visual_genome, refcocog, paco, fullanno, finecaption, use, prima, pascal_voc} have been strictly annotated to represent only the corresponding region in the caption. However, they fail to prevent duplicate captions from being assigned to multiple regions within the same image. Assigning a generic caption to multiple regions can lead to ambiguity in the association between regions and captions. Furthermore, these datasets primarily focus on salient regions, making models trained on them incapable of effectively handling multi-granularity regions. We argue that to generate truly unique captions for an image, it is crucial to consider multi-granularity masks and captions, as well as the global relationships between regions.

In this paper, we present \textit{\textbf{\ours}}, a multi-granularity captioning dataset designed to generate unique region-level captions with multi-granularity. Our objective is to create a dataset that includes regions at multiple granularities, providing diverse and unique captions. Unlike previous captioning datasets that are solely limited to salient regions within an image, our dataset covers a broader range of objects, parts, and backgrounds. Each caption in our dataset is uniquely mapped to a single region, ensuring a one-to-one correspondence between regions and captions across various granularities.
% To generate distinctive captions for regions while considering their relationships, we propose an automated data generation pipeline that annotates regions in a stage-wise manner using our mask tree structure. Mask tree contains the hierarchical relation of the regions in the mask. By leveraging the hierarchical structure, our automotive data pipeline easily generate unique caption for the target region regarding the tree node.
To generate unique captions for regions while considering their hierarchical relationships, we propose an automated data generation pipeline that annotates regions in a stage-wise manner using a \textit{mask tree} structure. The mask tree captures hierarchical dependencies by representing subset and superset relationships among regions. By leveraging this structure, our automated data pipeline efficiently generates unique captions for target regions based on their corresponding tree nodes.
Our dataset includes 0.001\% of SA-1B~\cite{sam} images and x\% aligned captions, specifically designed to train and evaluate unique captioning performance on multi-granularity regions.

Although previous models have demonstrated region understanding capabilities through various approaches, they still struggle to accurately capture given regions, particularly when dealing with multi-granularity regions~\cite{mug-vos}. Effectively handling multi-granularity regions requires encoding high-resolution features while preserving essential properties such as position and shape~\cite{finecaption}. However, existing models fall short in this aspect, making it difficult to fully utilize datasets like \textit{\textbf{\ours}}, which span a wide range of region sizes. To address these limitations, we propose \textbf{\model}, which effectively conditions regions of interest for the captioning model without losing the region's details. To achieve this, we implement mask encoder and dynamic mask modeling that extracts mask features while preserving essential properties such as position and shape even on the multi-granularity regions.

% Although previous captioning models have demonstrated region understanding capabilities through various approaches, they still struggle to accurately capture given regions, particularly when dealing with multi-granularity regions~\cite{mug-vos}. To address these limitations, we propose \textbf{\model}, which effectively conditions regions of interest for the captioning model without losing the region's details. To consider multi-granularity regions, it is essential to encode features from high resolution~\cite{finecaption}. To achieve this, we implement mask encoder and dynamic mask modeling that extracts mask features while preserving essential properties such as position and shape even on the multi-granularity regions.

To demonstrate the capability of \textbf{\textit{\model}} in generating unique multi-granularity region captions, we further validate our model on a test set that has undergone an additional quality assurance stage to ensure the quality of the annotated captions produced by our automated pipeline. Notably, \model achieves state-of-the-art performance on our \ours test set while also demonstrating strong performance on existing region-level captioning tasks using the Visual Genome~\cite{visual_genome} and RefCOCOg~\cite{refcocog} datasets.

\input{figs/previous_methods}

\input{tables/dataset_comparison}


In summary, our work makes the following key contributions:
\begin{itemize}
\item We introduce \textit{\textbf{\ours}}, a large-scale multi-granularity captioning dataset that ensures one-to-one region-caption mapping, covering a diverse range of objects, parts, and backgrounds beyond salient regions.
% \item We propose a novel automated data generation pipeline that leverages a stage-wise mask tree structure, enabling the creation of distinctive region captions while preserving global relationships within the image.
\item We present \textbf{\model}, a captioning model designed to handle multi-granularity regions through dynamic mask modeling and a high-resolution mask encoder that preserves essential region properties.
\item Extensive experiments demonstrate that \textbf{\model} achieves state-of-the-art performance on our \textbf{\ours} test set and shows strong generalization on traditional benchmark datasets, including Visual Genome and RefCOCOg.
\end{itemize}

==> sec/1_intro_jw.tex <==
\section{Introduction}
\label{sec:intro}
Multi-granularity region-level captioning, which involves describing any specific region in natural language, remains a challenging task. The key challenges of region-level captioning include effectively localizing the user-intended region~\cite{DenseCap, kosmos-2, glamm, Yu_2017_CVPR, osprey, controlcap, sca, omg-llava} and capturing its unique attributes~(e.g., color, relative position, and shape) to differentiate it from surrounding regions~\cite{wang2020uniqueinformativecaptioningimages, liu2019generating, wang2020compare}. Multi-granularity region-level captioning becomes even more challenging, as most prior studies have simply focused on salient regions of the scene failing to localize or describe smaller attributes.

Following the overwhelming success of Large Language Models (LLMs), previous approaches have explored the direction of utilizing Multi-Modal Large Language Models (MLLMs)~\cite{internvl-25, llava, improvedllava, arcana} for multi-granularity region-level captioning. Although they have demonstrated impressive results in region-level captioning, they still struggle to produce truly unique captions due to limitations in both model design and dataset availability.

Regarding model design, previous approaches~\cite{grit, flexcap, groma, gpt4roi} have explored regional captioning by providing region coordinates through natural language descriptions~\cite{llava, minigpt}, marking regions directly on the image (e.g., mask contours, ellipses, bounding boxes, triangles, scribbles, points, arrows, and masks)~\cite{vip-llava, yang2023finegrainedvisualprompting, shtedritski2023doesclipknowred}, or utilizing visual RoI features~\cite{regiongpt, omni-rgpt}. Although these methods have demonstrated notable performance, they come with several drawbacks: they may alter the original image, make it difficult to distinguish between colored contours, and fail to capture global relationships within the image~\cite{alpha-clip}, ultimately hindering the model's ability to generate unique captions.

On the other hand, we show that the na\"ive usage of existing captioning datasets~\cite{groma, osprey, glamm, visual_genome, refcocog, paco, fullanno, finecaption, use, prima, pascal_voc} is also problematic. Existing datasets include annotations that primarily focus on salient regions~\cite{}, preventing the model from successfully describing less salient properties. In addition, the majority of the captions are overly general~\cite{} (e.g., a person standing), leading to duplicate annotations that correspond to multiple regions within the same image. This prevents models from understanding and distinguishing similar regions, failing to faithfully describe the user-defined region.

To effectively overcome existing limitations, in this work, we first present a novel dataset \textit{\textbf{\ours}}, which is tailored for multi-granularity captioning. By utilizing existing Vision Language Models (VLMs)~\cite{internvl-25} and foundation models for instance segmentation~\cite{sam}, we propose an automated data generation pipeline consisting of multiple stages to create unique annotations that correspond to image regions in a one-to-one fashion. Unlike previous captioning datasets that are limited to salient regions within an image, our dataset covers a wide range of objects, parts, and backgrounds.

Based on our dataset, we then propose a novel model architecture \textbf{\model}, which effectively conditions regions of interest for the captioning model without losing the region's details. To consider multi-granularity regions, it is essential to encode features from high resolution~\cite{finecaption}. To achieve this, we introduce a mask encoder network and dynamic mask modeling approach that extracts mask features while preserving essential properties such as position and shape even on the multi-granularity regions.

To demonstrate the effectiveness of our proposed \textit{\textbf{\ours}} and \textbf{\textit{\model}} in generating unique multi-granularity region captions, we further validate our model on a test set that has undergone an additional quality assurance stage to ensure the quality of the annotated captions produced by our automated pipeline. Notably, \model achieves state-of-the-art performance on our \ours test set while also demonstrating strong performance on traditional region-level captioning datasets such as Visual Genome~\cite{visual_genome} and RefCOCOg~\cite{refcocog} datasets. We also show that further fine-tuning existing captioning models on \textit{\textbf{\ours}} enables better multi-granularity captioning.

\input{figs/previous_methods}

In summary, our work makes the following key contributions:
\begin{itemize}
\item We introduce \textit{\textbf{\ours}}, a large-scale multi-granularity captioning dataset that ensures one-to-one region-caption mapping by covering a diverse range of objects, parts, and backgrounds beyond salient regions.
% \item We propose a novel automated data generation pipeline that leverages a stage-wise mask tree structure, enabling the creation of distinctive region captions while preserving global relationships within the image.
\item We present \textbf{\model}, a captioning model designed to handle multi-granularity regions through dynamic mask modeling and a high-resolution mask encoder that preserves essential region properties.
\item Extensive experiments demonstrate that \textbf{\model} achieves state-of-the-art performance on our \textbf{\ours} test set and shows strong generalization on benchmark datasets, including Visual Genome and RefCOCOg.
\end{itemize}
